Improving Similar Language Translation With Transfer Learning

We investigate transfer learning based on pre-trained neural machine translation models to translate between (low-resource) similar languages. This work is part of our contribution to the WMT 2021 Similar Languages Translation Shared Task where we submitted models for different language pairs, including French-Bambara, Spanish-Catalan, and Spanish-Portuguese in both directions. Our models for Catalan-Spanish ($82.79$ BLEU) and Portuguese-Spanish ($87.11$ BLEU) rank top 1 in the official shared task evaluation, and we are the only team to submit models for the French-Bambara pairs.

==> stat_table.tex <==
\begin{table}[h]
\begin{center}
\textbf{Hi-Mr}
\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|} 
 \hline
\thead{\textbf{Language}} & \thead{\textbf{\#sentences}} & \thead{\textbf{\#words}} \\ 
 \hline
 \hline
hi & 43,274 & 829,976 \\
\hline
mr & 43,274 & 600,006  \\
\hline
mono-hi & 227,167,260 & 4,742,853,278  \\
\hline
mono-mr & 9,975,898 & 331,497,565 \\
\hline 
\hline
\end{tabular}
\textbf{Es-Ca}
\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|} 
 \hline
\thead{\textbf{Language}} & \thead{\textbf{\#sentences}} & \thead{\textbf{\#words}} \\ 
 \hline
 \hline
ca & 11,379,948 & 162,981,769 \\
\hline
es & 11,379,948 & 150,881,516  \\
\hline
mono-es & 58,416,064 & 1,525,007,410  \\
\hline
mono-ca & 24,745,986 & 763,697,712 \\
\hline 
\hline
\end{tabular}
\textbf{Es-Pt}
\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|} 
 \hline
\thead{\textbf{Language}} & \thead{\textbf{\#sentences}} & \thead{\textbf{\#words}} \\
es & 4,150,063 & 97,940,590 \\
\hline
pt & 4,150,063 & 94,756,496 \\
\hline
mono-es & 58,416,064 & 1,525,007,410  \\
\hline
mono-pt & 2,016,635 & 50,462,045 \\
\hline
\end{tabular}
\textbf{Sl-Hr}
\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|} 
 \hline
\thead{\textbf{Language}} & \thead{\textbf{\#sentences}} & \thead{\textbf{\#words}} \\
sl & 17,659,209 & 113,087,914  \\
\hline
hr & 17,659,209 & 117,736,580 \\
\hline
mono-sl & 46,251,729 & 770,646,199 \\
\hline
mono-hr & 64,577,734 & 1,244,102,908 \\
\hline
\end{tabular}
\textbf{Sl-Sr}
\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|} 
 \hline
\thead{\textbf{Language}} & \thead{\textbf{\#sentences}} & \thead{\textbf{\#words}} \\
sl & 14,130,116 & 79,135,558  \\
\hline
sr & 14,130,116 & 86,152,298 \\
\hline
mono-sl & 46,251,729 & 770,646,199 \\
\hline
mono-sr & 24,073,253 & 489,934,858 \\
\hline
\end{tabular}
\end{center}
\caption{\mam{It's odd to say ``A table showing\dots. You could say: ``Number of sentences\dots"} A table showing the number of sentences and words for the data used for each language pair.}\label{tab:data}
\end{table}
